Hadronic Vacuum Polarization and Test of Quantum Electrodynamics at Low Energies

A hadronic vacuum polarization correction to the photon propagator is found by using the Dubnicka-Meshcheryakov parameterization of the pion electromagnetic form factor and new experimental data on the $e^+e^-$ hadrons annihilation cross section. Then, the contribution from the hadronic vacuum polarization to the muon anomalous magnetic moment and the Lamb shift in muonic atoms are calculated.

==> title.tex <==
% Бош варақ
\thispagestyle{empty}
\begin{flushright}
\begin{tabular}{l}
\textbf{JOINT}\\
\textbf{INSTITUTE OF}\\
\textbf{NUCLEAR}\\
\textbf{RESEARCH}\\
\hspace{2.5cm}\textbf{DUBNA}	
\end{tabular}
\end{flushright}
\begin{flushleft}
	\includegraphics[scale=0.5]{logo-jinr.png}
\end{flushleft}
\hrule
\vspace{1.5cm}
\begin{flushright}
	\textbf{P2 -- 11308}
\end{flushright}
\vspace{2cm}
{\large
\hspace{2cm}\textbf{Gerdt V.~P., Karimkhodzhaev A., Faustov R.~N.}}
\vspace{2.5cm}

\hspace{1.6cm}\texttt{\Large HADRONIC VACUUM POLARIZATION}

\hspace{1.6cm}\texttt{\Large  AND TEST OF QUANTUM ELECTRODYNAMICS}

\hspace{1.6cm}\texttt{\Large AT LOW ENERGIES}

\vspace{3cm}
\begin{flushright}
	\textbf{\Huge 1978}
\end{flushright}
\hrule
\newpage
\thispagestyle{empty}
{\renewcommand{\thefootnote}{\fnsymbol{footnote}}
.
\vspace{8cm}
\begin{flushright}
	\textbf{P2 -- 11308}
\end{flushright}
\vspace{2cm}
{\large
\hspace{2cm}\textbf{V.P.GERDT}, \textbf{А.KARIMKHODZHAEV\footnote[1]{\textbf{\large INP AS UzSSR, Tashkent}}}, \textbf{R.N.FAUSTOV}}
\vspace{2.5cm}

\hspace{1.6cm}\texttt{\Large HADRONIC VACUUM POLARIZATION}

\hspace{1.6cm}\texttt{\Large AND TEST OF QUANTUM ELECTRODYNAMICS}

\hspace{1.6cm}\texttt{\Large AT LOW ENERGIES}

\vspace{3cm}

\hspace{1.6cm}\textit{\large \textbf{Sent to the collection ''Problems of the theory of gravitation}} 

\hspace{1.6cm}\textit{\large \textbf{and elementary particles ''}}}
\clearpage
